Efficient means of Achieving Composability using Object based Conflicts on Transactional Memory

Composing together the individual atomic methods of concurrent data-structures (cds) pose multiple design and consistency challenges. In this context composition provided by transactions in software transaction memory (STM) can be handy. However, most of the STMs offer read/write primitives to access shared cds. These read/write primitives result in unnecessary aborts. Instead, semantically rich higher-level methods of the underlying cds like lookup, insert or delete (in case of hash-table or lists) aid in ignoring unimportant lower level read/write conflicts and allow better concurrency. In this paper, we adapt transaction tree model in databases to propose OSTM which enables efficient composition in cds. We extend the traditional notion of conflicts and legality to higher level methods of cds using STMs and lay down detailed correctness proof to show that it is co-opaque. We implement OSTM with concurrent closed addressed hash-table(HT-OSTM)and list (list-OSTM) which exports the higher-level operations as transaction interface. In our experiments with varying workloads and randomly generated transaction operations, HT-OSTM shows speedup of 3 to 6 times and w.r.t aborts HT-OSTMis 3 to 7 times better than ESTM and read/write based STM, respectively. Where as,list-OSTM outperforms state of the art lock-free transactional list, NOrec STM list and boosted list by 30% to 80% across all workloads and scenarios. Further,list-OSTM incurred negligible aborts in comparison to other techniques considered in the paper.

==> optimizations.tex <==
\textbf{Optimization:} 
%\begin{enumerate}
If \npdel{} returns FAIL in \emph{\rvmt{} execution} phase then no need to validate it in \nptc{} (\emph{\upmt{} execution} phase). This is similar to the case of \npluk{} is being validated once. Since a failed \npdel{} \mth{} implies that it would not change the underlying \tab{} and in behaviour it is similar to a lookup as discussed in \figref{nostm32}.

\begin{figure}[H]
	\centering
	\captionsetup{justification=centering}
	%	\centering
	%\subfloat[H1 : Transactional tree histroy.]
	{\scalebox{0.5}{\input{figs/nostm32.pdf_t}}}
	\caption{Advantage of validating \npdel{} once, if its returning FAIL in \emph{\rvmt{} execution} phase}
	\label{fig:nostm32}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------------Garbage Collection---------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
%	\scriptsize
	\caption{\tabspace[0.2cm] gC($object\_list\downarrow$) : Garbage Collection.
		%\emph{DESCP}\tabspace: transvalidation of Tx.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $key$, $currs[]$, $val\_type$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $op\_status$ - OK or ABORT     
	}
	\label{algo:gc}
%	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{374}\makeatother
			\Function{gC}{} \label{lin:gc1}
			\cmntwa{to iterate over each hash-table object}
			\While{($obj\_{id}$ $\in$ $object\_list$)}
			\State j = 0;
			\cmntwa{to iterate over the each lazy skip list}
			\While{(j < size($obj\_{id}$))}
			\State head $\gets$ getLslHead($obj\_{id}$) \label{lin:gc2};
			\cmntwa{copy shared memory node}
			\State $pred$ $\gets$ \texttt{read(head)} \label{lin:gc3} ;
			\State $curr$ $\gets$ \texttt{read($pred.\rn$)}\label{lin:gc4};
			\While{($curr != tail$)}
			\cmntwa{live set is a concurrent Min Heap}
			\State $Min\_Tx$ $\gets$ \texttt{read}($getMin(LiveSet)$)\label{lin:gc5};
			\cmntwa{Min\_Tx monotonically increases}
			\If{((\texttt{read($curr.marked$)}) \& ($Min\_Tx$ $>=$ $(curr.max\_ts)))$}
			\State $pred.lock()$\label{lin:gc6};
			\State $curr.lock()$\label{lin:gc7};
			%\State $Min\_Tx.lock()$\label{lin:gc8}; \Comment{needed lock in case low TS Tx is added late to Live Set}
			\If{(validate\_gC($pred$, $curr$))}
			\State curr.deleted = true\label{lin:gc8.1};
			\State $pred.\rn$ $\gets$ $curr.\rn$ \label{lin:gc9};
			%  \State $pred.\bn$ $\gets$ $curr.\bn$ \label{lin:gc9}; \Comment{in case curr happens to be last marked node}
			\EndIf
			\State $pred.unlock()$\label{lin:gc10};
			\State $curr.unlock()$\label{lin:gc11};
			%  \State $Min\_Tx.unlock()$\label{lin:gc12};
			\EndIf
			\State $pred$ $\gets$ $curr$ \label{lin:gc13};
			\State $curr$ $\gets$ $curr.\rn$\label{lin:gc14};
			\EndWhile
			\State j++\label{lin:gc15};
			\EndWhile
			\EndWhile
			\State return $\langle \rangle$;
			\EndFunction 
		\end{algorithmic}
		
%	\end{multicols}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------------Validate Garbage Collection---------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
%	\scriptsize
	\caption{\tabspace[0.2cm] validate\_gC($pred\downarrow$, $curr\downarrow$) : Validate garbage collection.
		%\emph{DESCP}\tabspace: transvalidation of Tx.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $key$, $next[]$, $val\_type$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $op\_status$ - OK or ABORT     
	}
	\label{algo:vgc}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{406}\makeatother
		\Function{validate\_gC}{} \label{lin:vgc1}
		\If{($read$($curr.marked$ \& $pred.\rn$ = $curr$)}
		\State return $\langle TRUE\rangle$ \label{lin:vgc2};
		\EndIf
		\State return $\langle FALSE\rangle$ \label{lin:vgc3};
		\EndFunction 
	\end{algorithmic}
\end{algorithm}



\begin{enumerate}
	\item Need to lock $Min\_Tx$, because though the min\_Tx is always expected to increase but in case when multiple transactions begin simultaneously and the Tx with lower time stamp is slow and reaches late to Live set. In this case the Min\_tx will decrease. Figure showing this.
	\item Ensuring no duplicates would be inserted.
	\item Is there a guarantee that $Min\_Tx$ would only increase.
	\item When a node is deleted from \rn{} its deleted field is set True. and we depend on underlying gc mechanism to physically remove this node.
\end{enumerate}

